Foundations of Complex Event Processing

Complex Event Processing (CEP) has emerged as the unifying field for technologies that require processing and correlating distributed data sources in real-time. CEP finds applications in diverse domains, which has resulted in a large number of proposals for expressing and processing complex events. However, existing CEP languages lack from a clear semantics, making them hard to understand and generalize. Moreover, there are no general techniques for evaluating CEP query languages with clear performance guarantees. In this paper we embark on the task of giving a rigorous and efficient framework to CEP. We propose a formal language for specifying complex events, called CEL, that contains the main features used in the literature and has a denotational and compositional semantics. We also formalize the so-called selection strategies, which had only been presented as by-design extensions to existing frameworks. With a well-defined semantics at hand, we study how to efficiently evaluate CEL for processing complex events in the case of unary filters. We start by studying the syntactical properties of CEL and propose rewriting optimization techniques for simplifying the evaluation of formulas. Then, we introduce a formal computational model for CEP, called complex event automata (CEA), and study how to compile CEL formulas into CEA. Furthermore, we provide efficient algorithms for evaluating CEA over event streams using constant time per event followed by constant-delay enumeration of the results. By gathering these results together, we propose a framework for efficiently evaluating CEL with unary filters. Finally, we show experimentally that this framework consistently outperforms the competition, and even over trivial queries can be orders of magnitude more efficient.

==> compiling.tex <==
%!TEX root = ../main/main.tex

In this section we show how to compile a well-formed and unary CEL formula $\varphi$ into a CEA $\cA_\varphi$ that satisfies $\sem{\varphi}(S) = \sem{\cA_\varphi}(S)$ for every stream~$S$.
% Although we do not know how to efficiently evaluate CEA in general, we identify that an interesting fragment of (unary) CEL can be evaluated efficiently.
%In this section, we show how to compile CEL formulas into match automata towards having an efficient evaluation of CEL. 
Formally, we say that a CEL formula $\varphi$ is unary if for every subformula of $\varphi$ of the form $\varphi'\FILTER P(\bar{x})$, it holds that $P(\bar{x})$ is a unary predicate (i.e. $P(\bar{x}) \in \uset$).
For example, formulas $\varphi_1$, $\varphi_2$, and $\varphi_3$ in Section~\ref{sec:in_action} are unary, but formula $\varphi_4$ is not (the predicate $y.id = x.id$ is binary).
As motivated in Section~\ref{sec:in_action} and~\ref{sec:lp-normal-form} and further supported by our experiments (see Section~\ref{sec:experiments}), despite their appear simplicity unary formulas already present non-trivial computational challenges.

%MARTIN: ya lo dijimos
% The evaluation of full CEL is an interesting problem requiring new insights on rewriting techniques and more powerful computational models; we envision this as future work.

%For evaluating unary CEL formulas, we will follow an automata-based strategy: for each unary CEL formula $\varphi$ we will construct an equivalent CEA $\cA_\varphi$, and then use an efficient evaluation strategy for $\cA_\varphi$ to evaluate $\varphi$. 
%Formally, we say that a CEA $\cA$ is equivalent to a CEL formula $\varphi$ if $\sem{\varphi}(S) = \sem{\cA}(S)$ for every stream~$S$. Since we do not know how to efficiently evaluate $\cA_\varphi$ in general, we will show that an interesting subfragment of unary CEL can be evaluated efficiently.
%This will lead us to the first formal evaluation of~CEL. 
%Note that the construction of $\cA_\varphi$ will be done recursively from the syntactic structure of $\varphi$ and we will see the cost of each operation during the construction.

Now we present the compilation of unary core-CEL into CEA. The construction is closely related with the safeness condition and LP-normal form presented in Section~\ref{sec:language-prop}.
%Indeed, if a unary CEL safe formula $\varphi$ is in LP-normal form, one can convert $\varphi$ into a CEA in linear time. Unfortunately, if the safe formula is not in LP-normal form one has to afford an exponential blow-up in order to obtain the equivalent CEA.
\begin{theorem}\label{theo:core-automata}
	Given a well-formed formula $\varphi$ in unary core-CEL, there exists a CEA $\cA_\varphi$ equivalent to $\varphi$. Furthermore, $\cA_\varphi$ is of size at most linear in $|\varphi|$ if $\varphi$ is safe and in LP-normal form.

	%MARTIN: Esto sale gratis de los dos resultados anteriores y este.
	%, and of size at most double exponential in $|\varphi|$ otherwise.
\end{theorem} 
The proof of Theorem~\ref{theo:core-automata} goes by first converting $\varphi$ into an equivalent CEL formula $\varphi'$ in LP-normal form (Theorem~\ref{theo:LP-normal-form}) and then building an equivalent CEA from $\varphi'$. We show that there is an exponential blow-up for converting $\varphi$ into LP-normal form.
Furthermore, we show that the output of the second step is of linear size if $\varphi'$ is safe, and of exponential size otherwise. 
This shows that if we restrict the language to safe formulas, we can provide more efficient evaluation strategies for CEL.

We now study how to build CEA from CEL formulas with selection strategies. For this, we need to extend our framework and allow selection strategies to be applied directly over CEA.
Given a CEA $\cA$, a selection strategy $\SEL$ in $\{\sSTRICT,\sNEXT,\LAST,\sMAX\}$ and stream $S$, the set $\sem{\SEL(\cA)}(S)$ is defined analogously to $\sem{\SEL(\varphi)}(S)$ for a formula $\varphi$.
% For any stream $S$, we define $\sem{\SEL(\cA)}(S)$ to be the set of all matches $M$ such that $M \in \sem{\cA}(S)$ and $M$ is \emph{selected} by following the semantics of $\SEL$.
% A CEA $\cA_{\SEL}$ is equivalent to $\SEL(\cA)$ if $\sem{\SEL(\cA)}(S) = \sem{\cA_{\SEL}}(S)$ for every stream~$S$.

\begin{theorem}\label{theo:selectors-compilation}
	Let $\SEL$ be a selection strategy. For any CEA $\cA$, there is an CEA $\cA_{\SEL}$ equivalent to $\SEL(\cA)$. Furthermore, the size of $\cA_{\SEL}$ is, w.r.t. the size of $\cA$, at most linear if $\SEL=\sSTRICT$, and at most exponential otherwise.
\end{theorem}

At first the above result might seem unintuitive, specially in the case of $\sNEXT$, $\LAST$ and $\sMAX$. It is not immediate to show that there exists a CEA that can keep an unbounded number of different complex events with a finite number of states. However, this can be done with finite memory but with an exponential blow-up in the number of states.\par

Theorem~\ref{theo:selectors-compilation} concludes our study of the compilation of unary CEL into CEA. We have shown that CEA is not only able to evaluate CEL formulas, but also that it can be further exploited to evaluate selections strategies. In the next section we study how to evaluate CEA in practice.

% \martin{Creo que queda bien detenerse aquí y dejar lo de finitely ambiguous para la otra sección}

% Finally, the main disadvantage of these two operators is that the result is not necessarily finitely ambiguous and, therefore, we do not know how to evaluate $\cA_{\sSTRICT}$ and $\cA_{\sCEAX}$ efficiently.

% \martin{Este comentario quedó un poco en el aire, tengo que ver si lo muevo o lo elimino}


% We begin the discussion with the $\sNEXT$-operator, probably the most interesting and meaningful selection strategy for CEP-systems. At first sight, one could think that it is impossible to build a CEA for the $\sNEXT$-semantics: a CEA for computing the next semantics will have to remember and compare an unbounded number of matches which could lead to an unbounded amount of memory. Interestingly, this intuition is wrong since one can always build a CEA for computing the next semantics and, moreover, this construction has a very useful property.

% \begin{theorem}\label{theo:next-operator}
% 	Let $\cA$ be a CEA with $N$ states. Then, there is an $N$-ambiguous CEA $\cA_{\sNEXT}$ that is equivalent to $\NEXT(\cA)$ and of size at most exponential in the size of $\cA$.
% \end{theorem} 

% The previous result is very important for our framework, as one can always compute the next semantics of any CEA and, moreover, the resulting CEA is finitely ambiguous. Combined with Theorem~\ref{theo:UCEA-evaluation}, this leads to an efficient evaluation strategy for unary CEL formulas under the next semantics. 
% %The following corollary is probably the most important result of the paper.

% \begin{corollary}\label{theo:main-result}
% 	For every unary ecore-CEL formula $\varphi$, there is an efficient evaluation strategy for $\NEXT(\varphi)$. 
% 	Moreover, if $\cA_\varphi$ is a CEA equivalent to $\varphi$, the efficient evaluation strategy processes each event in time linear w.r.t. $\cA_\varphi$.
% \end{corollary} 
% This result guarantees that, if the $\sNEXT$-semantics is used over a unary CEL formula, one can efficiently evaluate the formula over any stream.
% Furthermore, the size of $\cA_{\sNEXT(\varphi)}$ is important for the performance of the evaluation.
% For this reason, Theorems~\ref{theo:core-automata} and~\ref{theo:extended-operators} must be considered to keep the construction as small as possible. 
% % Still, one has to notice that the automata constructions on Theorems~\ref{theo:core-automata},~\ref{theo:extended-operators} and~\ref{theo:next-operator} can be done \emph{on-the-fly}~\cite{gerth1996simple,Aho90,cox2007regular} over a CEL formula in LP-normal form and, thus, it is not needed to unfold the whole CEA $\cA_{\sNEXT(\varphi)}$ on memory in order to do the evaluation.
% For the final part of this section, we discuss how to compile the $\sSTRICT$ and $\sCEAX$ selection strategies. 
% In the following result, we show that both operators can be run by CEA.
% Unfortunately, they do not have the finitely ambiguous property as the $\sNEXT$-operator.

% \begin{theorem}\label{theo:strict-max-operators}
% 	For any CEA $\cA$, there are CEA $\cA_{\sSTRICT}$ and $\cA_{\sCEAX}$ equivalent to $\sSTRICT(\cA)$ and $\sCEAX(\cA)$, respectively. Further, $\cA_{\sSTRICT}$ ($\cA_{\sCEAX}$) is of size at most linear (double exponential, resp.) in the size of $\cA$.
% \end{theorem}


